Exploring the Intersection between Neural Architecture Search and Continual Learning

Despite the significant advances achieved in Artificial Neural Networks (ANNs), their design process remains notoriously tedious, depending primarily on intuition, experience and trial-and-error. This human-dependent process is often time-consuming and prone to errors. Furthermore, the models are generally bound to their training contexts, with no considerations to their surrounding environments. Continual adaptiveness and automation of neural networks is of paramount importance to several domains where model accessibility is limited after deployment (e.g IoT devices, self-driving vehicles, etc.). Additionally, even accessible models require frequent maintenance post-deployment to overcome issues such as Concept/Data Drift, which can be cumbersome and restrictive. By leveraging and combining approaches from Neural Architecture Search (NAS) and Continual Learning (CL), more robust and adaptive agents can be developed. This study conducts the first extensive review on the intersection between NAS and CL, formalizing the prospective Continually-Adaptive Neural Networks (CANNs) paradigm and outlining research directions for lifelong autonomous ANNs.

==> Sections/BiologicalBackground.tex <==
\section{Biological Background}

% \textit{Neuroplasticity} is one of the cornerstones to human intelligence, research in the field of Continual Learning has been focused on balancing the plasticity (the ability to acquire new information) and stability (the ability to retain existing knowledge) of an Artificial Neural Network. This trade-off is referred to as the \textit{stability-plasticity dilemma}.

% A step towards Artificial General Intelligence
%Although philosophically controversial and repeatedly criticized, the quest for a more human-like Artificial Intelligence (or Artificial General Intelligence (AGI)) is still considered the ultimate goal of research in AI \cite{baum_2010}.

% Learning and Memory are the foundation of intelligence
Human intelligence is contingent on the acquisition and consolidation of knowledge; research in the field of Evolutionary Neuropsychology has revealed that the majority of the evolutionary advances our species has accomplished are founded upon associative learning and memory \cite{coolidge_2020}. \textit{Synaptic Plasticity}, or the ability to change synapses' strengths, is thought to underlie both the learning and memory mechanisms in mammalian brains \cite{takeuchi_2014,feldman_2020}.

% Briefly mention that there are types of Non-Synaptic Plasticity
% While Synaptic Plasticity is crucial to human intelligence, it is certainly not the only form of neural plasticity \cite{abraham_2019}. One type of \textit{Non-Synaptic Plasticity} is \textit{Intrinsic Plasticity} (IP), or \textit{Intrinsic Neuronal Excitability}. IP allows neurons themselves to have adaptive qualities pertaining to their electrical properties due to neuronal and synaptic activities, which plays an essential role in maintaining homeostasis \cite{oleary_2014}. Both Synaptic and Non-Synaptic Plasticity together allow our brains to perform complex tasks, such as learning, thinking, and retaining memories \cite{sehgal_2013,tully_2014}.

% Section outline
In this section, we conduct a brief review on Associative Learning, Memory Formation and Retention, and the \textit{Complementary Learning Systems} (CLS) in biological neural networks.


\subsection{Associative Learning}

% Synaptic Potentiation
One of the cornerstones of Biological (as well as Computational) Neuroscience is the Hebbian learning rule, postulated by Donald Hebb in 1949 \cite{hebb_1949}. The premise behind the rule is that the learning process in biological neural networks is activity-dependent. If a pre-synaptic neuron A is repeatedly successful in activating a post-synaptic neuron B, the strength of the synapse will gradually increase (also referred to as \textit{Synaptic Potentiation}), which henceforth provides the basis for associative learning. 

% Synaptic Potentiation + STDP
Hebb's theory is often inaccurately summarized as the mnemonic "neurons that fire together, wire together", which can be misleading as the neurons in this context do not activate simultaneously. Temporal precedence is imperative for Synaptic Potentiation to occur; the pre-synaptic neuron must be excited strictly \textit{prior} to the post-synaptic neuron's activation. This emphasis on the timing of neuronal activity foreshadowed a form of Synaptic Plasticity called \textit{Spike-Timing Dependent Plasticity} (STDP), which is considered the underlying mechanism for the Hebbian learning model as well as information storage \cite{park_2017,susman_2019}.

% Flaw in Hebb's postulate
% While Hebb's postulate is widely considered the foundation of Machine Learning, it had a fundamental flaw that was not addressed for nearly three decades. The most basic form of Hebbian learning is modelled as the product of the pre- and post-synaptic activities, regulated by a learning rate $\eta$:

% \begin{equation}
% \Delta W_{ab} = \eta X_{a} \cdot Y_{b}
% \label{eq:hebbian_learning_model}
% \end{equation}

% Explaining how Hebb's equation is monotonically increasing with no upper-bound or regulatory terms
% Since $\eta,X_{a},Y_{b} \geq 0$, the change in synaptic strength $\Delta W_{ab}$ will always be positive and therefore Equation (\ref{eq:hebbian_learning_model}) represents a monotonically increasing function that eventually leads to unstable, runaway neuronal activity.

% Synaptic Depression
% It was not until 26 years later that Gunther Stent appended a regulatory definition to Hebb's theory to prevent the perpetual potentiation of synapses \cite{stent_1973}. The mechanism for \textit{Synaptic Depression}, or the weakening of synaptic efficacy, borrows from the causality aspect of Synaptic Potentiation: if neuron A consistently does not take part in firing neuron B, synapse $W_{ab}$ weakens. This new rule pertaining to synaptic weakening due to lack of co-occurring activity led to the popular adage "use it or lose it".

% Homeostatic Plasticity through IP
% In addition to Stent's appendage, \textit{Homeostatic Plasticity} of neuronal excitation persistently regulates the activation of neurons through Intrinsic Plasticity and several other means \cite{apostolopoulou_2020}. While Hebbian Plasticity is responsible for the potentiation or depression of synapses, Homeostatic Plasticity attempts to modulate and maintain the neurons' original states, or "homeostasis", through the intrinsic properties of the neurons \cite{fox_2017,zhang_2019}.

% Neuromodulation 
Another mean to further control and stabilize neuronal activity is through \textit{Neuromodulation}, which is the process of altering the neuron's intrinsic firing activity through chemical modulators. The most effective neuromodulators on learning and memory are thought to be dopamine (DA), serotonin (5-HT), acetylcholine (ACh), and noradrenaline (also called norepinephrine (NE)) \cite{palacios-filardo_2019,bazzari_2019}. These modulators (specifically dopaminergic and serotonergic neuromodulation) have been observed to decline in adults, which diminishes their reward-based learning and decision-making skills \cite{eppinger_2011}. These numerous and distinct factors, each affecting the changes in synaptic efficacy in different ways, are vital to the stability of neuronal activity and facilitate the complex mechanisms that underlie intelligence.

% Introducing our synaptic plasticity taxonomy
% Synaptic Plasticity can occur through 2 different means: \textit{Homosynaptic Plasticity} and \textit{Heterosynaptic Plasticity}, which are less often referred to as synaptic \textit{Intrinsic Plasticity} (not to be confused with the previously discussed neuronal Intrinsic Plasticity) and \textit{Extrinsic Plasticity} \cite{chistiakova_2014}.

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.45\textwidth]{Images/synaptic_plasticity_types.eps}
% \caption{Types of Synaptic Plasticity}
% \label{fig:synaptic_plasticity_types}
% \end{figure}

% Explaining homo-/hetero-synaptic plasticity
% If a change in synaptic strength takes place due to consecutive activity in the pre- and post-synaptic neurons (neuron A and B in Figure (1), respectively), it is considered a result of Homosynaptic Plasticity. Whereas if the change in synaptic efficacy is caused by a different path (a change in $W_{cb}$ due to stimulation in A), it is categorized as Heterosynaptic Plasticity.


\subsection{Memory Formation and Retention}

% Memory is a more challenging/complex framework than learning
Although Associative Learning in biological neural networks is a considered relatively intuitive model, the mechanism underlying memory is significantly more complex and is thought to be one of the most compelling and challenging research areas in the field of Neuroscience \cite{lynch_2004,dringenberg_2020}. It is worth noting that researches on cognitive psychology have revealed that memory entails a learning process in itself \cite{tulving_1995}, and thus the mechanisms for both processes are interleaved.

% Theory: the huge number of dendrites facilitate memory
% Some studies hypothesized that due to the sheer number of dendrites in every neuron, a masking mechanism naturally occurs that allows most synapses associated with past experiences to be mostly left untouched whilst only a subset of the connections are allocated to learning new information \cite{hawkins_2016}. 

% Introducing temporal taxonomy of synaptic plasticity
The types of Synaptic Plasticity can be categorized according to the locality of the signals (Homo/Hetero-Synaptic Plasticity \cite{chistiakova_2014}) or the temporal qualities of the neural activation (i.e how long the signal lasts). Studies on \textit{Long-Term Synaptic Plasticity} and \textit{Short-Term Synaptic Plasticity} have unveiled an undeniable association between the temporal type of Synaptic Plasticity and memory formation \cite{citri_2007}.

\begin{figure}[H]
\centering
\includegraphics[width=0.48\textwidth]{Images/synaptic_plasticity_temporal_types_alt.eps}
\caption{Temporal types of Synaptic Plasticity}
\label{fig:synaptic_plasticity_temporal_types}
\end{figure}

% LTP
Long-Term Potentiation (LTP) is considered the most studied branch of Synaptic Plasticity \cite{abraham_2019}; ever since its formal description in 1973, it has attracted an increasing attention in the neuroscience research community, especially in relation to learning and the cellular models of memory \cite{lomo_1973,escobar_2007,wiegert_2013,dringenberg_2020}. % LTP is thought to have both Homo- and Hetero-synaptic components and is caused by persistent strengthening of the synapse over longer periods of time. 
While there has not been any conclusive proof that memory resides in the synapses and that it is possibly a result of non-synaptic mechanisms \cite{abraham_2019}, numerous studies strongly support the theory that LTP within the hippocampus is at least partially responsible for learning and for the formation and retention of memory \cite{barnes_1979,dringenberg_2020,deperrois_2020}.

% LTD
Intuitively, it is thought that a particularly strong connections between a set of neurons that resulted from high-frequency, persistent strengthening of synapses is a direct representation of memory on a cellular level. On the other hand, lack of access to those memories would result in hippocampal \textit{Long-Term Depression}, which is the weakening of synapses, causing a gradual decay of unused memories over time \cite{tsumoto_1993,escobar_2007}. Some studies suggest that in the context of developing brains, LTD in already weakened synapses might result in synaptic pruning, which indicates that Long-Term Synaptic Plasticity plays a prominent role in the development of the neural structure \cite{lynch_2004,wiegert_2013,piochon_2016}. As the brain ages, however, plasticity decays and the brain becomes less prone to drastic changes \cite{hensch_2004,oberman_2013}.

% STF / STD / PTP
Short-Term Synaptic Plasticity, in contrast, refers to the changes in synaptic efficacy that can only last in the order of tens to thousands of milliseconds \cite{regehr_1970}. There are 3 main categories of Short-Term Synaptic Plasticity: \textit{Short-Term Facilitation} (STF), \textit{Augmentation} or \textit{Post-Tetanic Potentiation} (PTP), and \textit{Short-Term Depression} (STD) \cite{regehr_1970}. The short-term counterparts of LTP and LTD are STF and STD, respectively. While the exact impact of Short-Term Synaptic Plasticity on memory and learning is not yet conclusive, it is thought to have a similar effect as Long-Term Synaptic Plasticity, but on relevant timescales \cite{stevens_1995,markram_1996}. Post-Tetanic Potentiation is also a short-lived increase in the synapses' strength as a result of repetitive, high-frequency stimulus. Some studies suggest that hippocampal PTP is responsible for short-term memory \cite{vandael_2020}.

% Neurogenesis and memory
% Another interesting hypothesis relating to memory-creation and consolidation is through \textit{Neurogenesis}, which is the generation of new neurons from neural stem cells. Neurogenesis is considered a crucial process in developing brains (embryos in particular), and as with other forms of plasticity, it decays over time \cite{urban_2014}. Some studies, however, suggest that Neurogenesis still occurs in adult brains (albeit at a much lower rate \cite{sorrells_2018}) and that when new neurons are integrated into certain parts of the hippocampus, they can be directly related to the formation of new memories \cite{deng_2010}. Similar to Neurogenesis, research suggests that newly-developed synapses and synaptic circuits have also been observed in relation to acquiring new memories \cite{lynch_2004,kennedy_2013}.


\subsection{The Complementary Learning Systems}

% Explaining the Hippocampus'/Neocortex's effects on learning/memory
The Complementary Learning Systems framework, which was articulated by McClelland et al. in 1995, defines the distinct roles of the mammalian hippocampal and neocortical systems on learning and episodic memory \cite{mcclelland_1995}. The theory holds that the hippocampus is responsible for rapid learning and retaining short-term, sparse memories, which can later be replayed to the neocortex for more efficient encoding and long-term storage. Although the CLS is characterized as a theory, it has had over 25 years' worth of empirical data generally supporting its premise \cite{oreilly_2011,blakeman_2020}.

While the hippocampus facilitates the fast and arbitrary episodic learning and memory formation/retrieval, the neocortex (specifically the Prefrontal Cortex (PFC)) tends to be responsible for long-term preservation and recall of memory \cite{funahashi_2007}. Some studies have shown that new memories get encoded in both the hippocampal and neocortical systems simultaneously; the hippocampus would be responsible for short-term recall, and over time the PFC would consolidate the memory and take-over the retrieval duty \cite{kitamura_2017}. 

% Memory and sleep
Numerous studies found compelling evidence that the consolidation of memories from the hippocampus to the PFC occurs during various stages of sleep \cite{marshall_2007,langille_2019}. While a subject is awake, the hippocampus' rapid-encoding capabilities accommodate the fact-paced acquisition of information, which are then slowly learned by the PFC and encoded in an overlapped and compressed manner during sleep \cite{schapiro_2017}. Other researches theorize that in addition to memory consolidation, brains tend to also organize and selectively forget older memories during sleep \cite{langille_2019}.

% The CLS and Hebbian learning
% To varying degrees, both the hippocampus and the neocortex are thought to rely on Hebbian learning due to their tendency to bind co-occurring features of an experience (an episode) together \cite{oreilly_2000}. The hippocampus, more so than the neocortex, is universally assumed to use a Hebbian form of learning, given that short-term memories are thought to share the localized Hebbian nature of proximity-based neural correlated activities \cite{ketz_2013}.

% Transition to Continual Learning
These theoretical models that capture our innate ability to retain important knowledge while gradually forgetting rarely accessed information have inspired numerous computational models, leading to the emergence of the Continual Learning paradigm.

==> Sections/To_do.tex <==

% NOTES

% "Learning and plasticity are thus central to consciousness" \cite{cleeremans_2011}


Intro to RL NAS subsubsection, make sure the controller network is the agent

First paragraph of Lower Fidelity Estimation should be rewritten to have less awkward grammar.

% Assume multi-modality in PANNs?

CL autonomous bootstrapping technique;  most CL algorithms must have explicitly separate tasks (e.g: gating mechanism-based CL)

Add column to NAS table for Hyperparameter Optimization (checkmarks)

Add human expert models (resnet/densenet/inceptionnet) to NAS table (maybe?)



% General Notes

Continual Data-prep = takes into account previous knowledge to collect relevant data (similar data distributions), feature engineering (normalize images, downsample etc...) similar to previous data, synthesize new data to boost performance of model.

Add more eqs or Lemmas (inspiration in One-Shot NAS overcoming catastrophic forgetting ieee paper)


Mention Weight Plasticity Loss (WPL, \cite{zhang_E2NAS_2020,pasunuru_2019}) in CL section Prior-Focused part.

Single vs multihead incremental learning in cl section

Add MO to NAS table

==> TablesAndPseudocode/PANNModelsTable.tex <==
% \renewcommand{\arraystretch}{2.25}
% \begin{table*}[!ht]
%     \centering
%     \rowcolors{0}{}{gray!5}
%     \begin{tabular}{M{3cm} M{2.5cm} M{2.5cm} M{0.2cm} M{2.5cm} M{2.5cm} M{2cm}}
%         \toprule
%         Reference / Model & \multicolumn{2}{c}{PANN Component(s)} && \multicolumn{2}{c}{Memory-Retention Strategy} & Optimization Approach \\
%         \midrule
        
%          % Lüders et al. (ENTM) \cite{luders_2016} & Model Plasticity & Neural Architecture && Parameter-Constraint & Parameter Isolation & EA \\
         
%          % Yang et al. \cite{yang_2018} & Data & Data Collection && - & - & - \\
         
%          Li et al. (Learn-to-Grow) \cite{li_2019} & Model Plasticity & Neural Architecture && Parameter-Constraint & Prior-Focused \& Parameter Isolation & GO \\
         
%          Huang et al. (CNAS) \cite{huang_2019} & Model Plasticity & Neural Architecture && Replay-Based & Episodic Rehearsal & RL \\
         
%          Pasunuru \& Bansal \cite{pasunuru_2019} & Model Plasticity & Neural Architecture && Parameter-Constraint & Prior-Focused & RL \\
         
%          Zhang et al. (E$^{2}$NAS) \cite{zhang_E2NAS_2020} & Model Plasticity & Neural Architecture && Parameter-Constraint & Prior-Focused & GO \\
         
%          Zhang et al. (REC) \cite{zhang_rec_2020} & Model Plasticity & Neural Architecture \& Hyperparameters && Parameter-Constraint & Data- \& Prior-Focused & RL \\
         
%          Du et al. (ENAS-S) \cite{du_2021} & Model Plasticity & Neural Architecture && Parameter-Constraint & Parameter Isolation & EA \\
         
%          Niu et al. (AdaXpert) \cite{niu_2021} & Model Plasticity & Neural Architecture && Paramater-Constraint & Data-Focused & RL \\
         
%          Zhang et al. \cite{zhang_2021} & Model Plasticity & Neural Architecture && Parameter-Constraint & Prior-Focused & RS \\
         
%          Qin et al. (BNS) \cite{qin_2021} & Model Plasticity & Neural Architecture && Replay-Based & Episodic Rehearsal & RL \\
         
%          Mundt et al. (DP-NAS) \cite{mundt_2021} & Model Plasticity & Neural Architecture && Replay-Based & Generative Rehearsal & RL \\
         
%          Gao et al. (CLEAS) \cite{gao_2022} & Model Plasticity & Neural Architecture \& Hyperparameters && Parameter-Constraint & Parameter Isolation & RL \\
         
         
%         \bottomrule
%     \end{tabular}
%     \bigskip
%     \caption{Existing Partially-Plastic ANNs}
%     \label{tab:pann_models}
% \end{table*}


\begin{table*}[!htp]
    \centering
    \rowcolors{0}{}{gray!5}
    \begin{tabular}{M{3cm} M{1.5cm} M{2.25cm} M{2.25cm} M{2.5cm} M{2.25cm} M{1.25cm}}
        \toprule
        Reference / Model & Optimization Approach & Plasticity Type & \multicolumn{2}{c}{Memory-Retention Strategy} & Benchmark & \makecell{Error \\ (avg. \%)} \\
        \midrule
        
         \makecell{Li et al. 2019 \\ (Learn-to-Grow) \cite{li_2019}} & GO & Neural Architecture & Parameter-Constraint & Prior-Focused \& Parameter Isolation & \makecell{ImageNet, \\ CIFAR100, \\ + 8 others (avg)} & \makecell{30.16, \\ 20.41, \\ 22.32 } \\
         
         \makecell{Huang et al. 2019 \\ (CNAS) \cite{huang_2019}} & RL & Neural Architecture & Replay-Based & Episodic Rehearsal & \makecell{MNIST, \\ Fashion MNIST} & \makecell{1.96, \\ 7.26} \\
         
         \makecell{Pasunuru \& Bansal 2019 \\ (CAS) \cite{pasunuru_2019}} & RL & Neural Architecture & Parameter-Constraint & Prior-Focused & \makecell{MSR-VTT, \\ MSVD } & \makecell{55.50, \\ 38.30} \\
         
         \makecell{Zhang et al. 2020 \\ (E$^{2}$NAS) \cite{zhang_E2NAS_2020}} & GO & Neural Architecture & Parameter-Constraint & Prior-Focused & \makecell{CIFAR10, \\ CIFAR100, \\ ImageNet16} & \makecell{6.11, \\ 27.95, \\ 34.33} \\
         
         \makecell{Zhang et al. 2020 \\ (REC) \cite{zhang_rec_2020}} & RL & Neural Architecture \& Hyperparameters & Replay-Based \& Parameter-Constraint & Episodic Rehearsal \& Prior-Focused & \makecell{Permuted MNIST, \\ MNIST Variation, \\ CIFAR100} & \makecell{4.30, \\ 28.50, \\ 40.30} \\
         
         \makecell{Wu et al. 2020 \\ (Firefly) \cite{wu_2020}} & MO & Neural Architecture & Parameter-Constraint & Parameter Isolation & \makecell{CIFAR100} & \makecell{8.97} \\
         
         \makecell{Du et al. 2021 \\ (ENAS-S) \cite{du_2021}} & EA & Neural Architecture & Parameter-Constraint & Parameter Isolation & \makecell{CIFAR10, \\ CIFAR100} & \makecell{-, \\ 26.5} \\
         
         \makecell{Niu et al. 2021 \\ (AdaXpert) \cite{niu_2021}} & RL & Neural Architecture & Paramater-Constraint & Data-Focused & \makecell{ImageNet100, \\ ImageNet1000} & \makecell{19.26, \\ 18.87} \\
         
         \makecell{Zhang et al. 2021 \\ (NSAS) \cite{zhang_2021}} & RS & Neural Architecture & Parameter-Constraint & Prior-Focused & \makecell{CIFAR10, \\ CIFAR100, \\ ImageNet16} & \makecell{6.45, \\ 29.31, \\ 57.86} \\
         
         \makecell{Qin et al. 2021 \\ (BNS) \cite{qin_2021}} & RL & Neural Architecture & Replay-Based & Episodic Rehearsal & \makecell{MNIST, \\ CIFAR10, \\ CIFAR100} & \makecell{0.13, \\ 8.60, \\ 17.61} \\
         
         \makecell{Mundt et al. 2021 \\ (DP-NAS) \cite{mundt_2021}} & RL & Neural Architecture & Replay-Based & Generative Rehearsal & \makecell{MNIST, \\ CIFAR10} & \makecell{23.61, \\ 34.85} \\
         
         \makecell{Gao et al. 2022 \\ (CLEAS) \cite{gao_2022}} & RL & Neural Architecture \& Hyperparameters & Parameter-Constraint & Parameter Isolation & \makecell{Permuted MNIST, \\ Rotated MNIST, \\ CIFAR10 } & \makecell{3.70, \\ 3.00, \\ 33.10} \\
         
         
        \bottomrule
    \end{tabular}
    \bigskip
    \caption{Existing Partially-Plastic ANNs}
    \label{tab:pann_models}
\end{table*}

